Conditional [MASK] Discrete Diffusion Language Model

Although auto-regressive models excel in natural language processing, they often struggle to generate diverse text and provide limited controllability. Non-auto-regressive methods could be an alternative but often produce degenerate outputs and exhibit shortcomings in conditional generation. To address these challenges, we propose Diffusion-EAGS, a novel framework that integrates conditional masked language models into diffusion language models through the theoretical lens of a conditional Markov Random Field. In doing so, we propose entropy-adaptive Gibbs sampling and entropy-based noise scheduling to counterbalance each model's shortcomings. Experimental results show that Diffusion-EAGS outperforms baselines and achieves the best quality-diversity tradeoff, demonstrating its effectiveness in non-autoregressive text generation.

==> 09_conclusion.tex <==

In this work, we introduce Diffusion-EAGS, integrating PLMs with diffusion models for conditional generation. By leveraging step-wise diffusion models and the property of MLM, we demonstrate that MLM-based PLMs can serve as denoising function with Entropy-based Adaptive Gibbs Sampling. We also propose entropy-based noise scheduling during training for adaptive sampling. Experimental results demonstrate that Diffusion-EAGS outperforms existing baselines, yielding improved text generation quality, enhanced diversity, broad applicability, and more precise token-level control.



==> fig/analfigs.tex <==
\begin{figure*}[h]
\centering
\subfigure[]{\includegraphics[width=.65\columnwidth]{fig/pareto_chart.png}
\label{fig:pareto}}
\subfigure[]{\includegraphics[width=.65\columnwidth]{fig/sentence_entropy_plot_v2.png}
\label{fig:entropy}}
\subfigure[]{\includegraphics[width=.65\columnwidth]{fig/sat_deon1.png}
\label{fig:sat_deontology}}
\caption{
(a) Average reconstruction error as a function of the number of groups.
(b) Average reconstruction errors of ten scenarios.
}
\end{figure*}

==> tab/tab5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}



\begin{table}[h]
\centering
\vspace*{-0.4cm}
\resizebox{\linewidth}{!}{%
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l ll}
\specialrule{0.5pt}{0pt}{0pt} \hline
                         % \multicolumn{3}{c}{Sentence}                                                   \\ \hline
\multicolumn{2}{l}{\multirow{2}{*}{Context}}                       & Jake was playing with his toys. He accidentally broke his favorite one.         \\
\multicolumn{2}{l}{}                                               & He cried a lot over it. His parents decided to replace it for him.              \\ \hline
\multirow{2}{*}{Keyword } & \multicolumn{1}{c}{not stop}    & Jake just could \textbf{not stop} crying.                                               \\
                         &  \multicolumn{1}{c}{Jake feel}   & It made \textbf{Jake feel} So much better.                                              \\
                          \specialrule{0.5pt}{0pt}{0pt} \hline
\end{tabular}
}
\vspace*{-0.3cm}
\caption{Keyword-based Generation}
\vspace*{-0.5cm}
\label{tab:keyword_gen}
\end{table}
